Graph Structure Learning with Variational Information Bottleneck

Graph Neural Networks (GNNs) have shown promising results on a broad spectrum of applications. Most empirical studies of GNNs directly take the observed graph as input, assuming the observed structure perfectly depicts the accurate and complete relations between nodes. However, graphs in the real world are inevitably noisy or incomplete, which could even exacerbate the quality of graph representations. In this work, we propose a novel Variational Information Bottleneck guided Graph Structure Learning framework, namely VIB-GSL, in the perspective of information theory. VIB-GSL advances the Information Bottleneck (IB) principle for graph structure learning, providing a more elegant and universal framework for mining underlying task-relevant relations. VIB-GSL learns an informative and compressive graph structure to distill the actionable information for specific downstream tasks. VIB-GSL deduces a variational approximation for irregular graph data to form a tractable IB objective function, which facilitates training stability. Extensive experimental results demonstrate that the superior effectiveness and robustness of VIB-GSL.

==> 3_preliminary.tex <==
\section{Notations and Preliminaries}
% Graph structure learning
% \subsection{Problem Definition}
Let $\{(G_1, Y_1), (G_2, Y_2), \dots, (G_N, Y_N)\}$ be a set of $N$ graphs with their labels. 
We denote $G_n$ as the $n$-th graph with node set $V=\{v_i, i=1,2,\dots, M\}$, node feature matrix $X\in\mathbb{R}^{M\times d_0}$ of $V$ with $d_0$ dimensions, and adjacency matrix $A\in\mathbb{R}^{M\times M}$. 

We will use the following standard quantities in the information theory~\cite{cover1999elements} frequently:
Shannon entropy $H(X)=\mathbb{E}_{X\sim p(X)}[-\log p(X)]$, cross entropy $H(p(X),q(X))=\mathbb{E}_{X\sim p(X)}[-\log q(X)]$, Shannon mutual information $I(X,Y)=H(X)-H(X|Y)$, and Kullback Leiber divergence $\mathcal{D}_{\rm KL}(p(X)||q(X)=\mathbb{E}_{X\sim p(X)}\log\frac{p(X)}{q(X)}$. 
\subsection{Graph Structure Learning}
Given a graph $G=(X, A)$ with feature matrix $X$ and adjacency matrix $A$, or only given a feature matrix $X$, the graph structure learning problem we consider in this paper can be formulated as producing an optimized graph $G^*=(X, A^*)$ and its corresponding graph representation $Z^*=f(G^*)$, with respect to the graph-level tasks. 

% \subsection{Graph Information Bottleneck}
\subsection{Information Bottleneck}
Following standard practice in the IB literature~\cite{tishby2000information}, given data $X$, representation $Z$ of $X$ and target $Y$, $(X,Y,Z)$ are following the Markov Chain $<Y\to X \to Z>$. 
\begin{myDef}[Information Bottleneck]
For the input data $X$ and its label $Y$, the the \textbf{Information Bottleneck} principle aims to learn the minimal sufficient representation $Z$:
\begin{equation}
    Z = \arg\min_{Z}-I(Z, Y)+\beta I(Z, X),
\end{equation}
where $\beta$ is the Lagrangian multiplier trading off sufficiency and minimality. 
\end{myDef}

\cite{alemi2016deep} proposed a tractable lower bound of  the IB objective for deep neural networks:
\begin{equation}
\begin{aligned}
    \mathcal{L}=\frac{1}{N}\sum^{N}_{i=1}\int &dZp(Z|X_i)\log q(Y_i|Z)\\
    &+\beta \mathcal{D}_{KL}\left(p(Z|X_i),r(Z)\right),
\end{aligned}
\end{equation}
% \begin{equation}
%     \mathcal{L}=\frac{1}{N}\sum^{N}_{i=1}\int dZp(Z|X_i)\log q(Y_i|Z)+\beta \mathcal{D}_{KL}(p(Z|X_i),r(Z)),   
% \end{equation}
where $q(Y_i|Z)$ is the variational approximation to $p(Y_i|Z)$ and $r(Z)$ is the variational approximation of $Z$'s prior distribution. 
% \subsection{Graph Information Bottleneck}
% \begin{myDef}[Graph Information Bottleneck]
% For a graph $G$ and its label $Y$, the \textbf{Graph Information Bottleneck} aims to seek for the most informative yet compressed representation $Z$ following the Markov chain $<Y\to G \to Z>$:
% \begin{equation}
%     Z = \arg\min_{Z}-I(Z, Y)+\beta I(Z, G),
% \end{equation}
% where $\beta\ge 0$ is the Lagrangian multiplier trading off sufficiency and minimality and $I(\cdot,\cdot)$ is the mutual information. 
% \end{myDef}
